WorldSimBench: Towards Video Generation Models as World Simulators

Recent advancements in predictive models have demonstrated exceptional capabilities in predicting the future state of objects and scenes. However, the lack of categorization based on inherent characteristics continues to hinder the progress of predictive model development. Additionally, existing benchmarks are unable to effectively evaluate higher-capability, highly embodied predictive models from an embodied perspective. In this work, we classify the functionalities of predictive models into a hierarchy and take the first step in evaluating World Simulators by proposing a dual evaluation framework called WorldSimBench. WorldSimBench includes Explicit Perceptual Evaluation and Implicit Manipulative Evaluation, encompassing human preference assessments from the visual perspective and action-level evaluations in embodied tasks, covering three representative embodied scenarios: Open-Ended Embodied Environment, Autonomous, Driving, and Robot Manipulation. In the Explicit Perceptual Evaluation, we introduce the HF-Embodied Dataset, a video assessment dataset based on fine-grained human feedback, which we use to train a Human Preference Evaluator that aligns with human perception and explicitly assesses the visual fidelity of World Simulators. In the Implicit Manipulative Evaluation, we assess the video-action consistency of World Simulators by evaluating whether the generated situation-aware video can be accurately translated into the correct control signals in dynamic environments. Our comprehensive evaluation offers key insights that can drive further innovation in video generation models, positioning World Simulators as a pivotal advancement toward embodied artificial intelligence.

==> sec/1_intro.tex <==
\begin{figure}[h]
\begin{center}
\includegraphics[width=1\linewidth]{ICLR_2025_WorldSimBenchmark/fig/motivation.pdf}
\end{center}
\caption{(Left)~Overview of the hierarchical capabilities of the Predictive Generative Model. \mname ~evaluates Predictive Generative Models up to $S_3$, and these models are also referred to as World Simulators. \mname ~assesses the models from the perspectives of video generation and action transformation. (Center)~Overview of the 22 evaluation dimensions across three embodied scenarios in \upstream. (Right)~Overview of the 20 embodied evaluation tasks across the same three scenarios in \downstream. Completing a \downstream task implicitly involves evaluating multiple \upstream dimensions. 
% For example, the robotic arm task of 'grasping the blue block' requires the generated video to exhibit accurate trajectory and object interaction attributes. Thus, we constructed \mname, a hierarchical evaluation framework that integrates both \downstream and \upstream assessments to comprehensively evaluate the World Simulator.
\zhelun{delete object deformation and hallucination, change to three dimes, redraw}} 
\label{fig:motivation}
\end{figure}




\section{Introduction \textbf{major review@yiran}}

Before taking action, humans make predictions based on their objectives and observations of the current environment. 
%
These predictions manifest in various forms, such as textual planning, visual imagination of future scene changes, or even subconscious planning at the action level. 
%
Each of these predictive capabilities is critical to the successful completion of tasks. 
%
We anticipate that future embodied agents, driven by predictive generative models, will need to exhibit similar capabilities. 
%
Recently, with the advancement of Large Language Models (LLMs)~\cite{} and Multimodal Large Language Models (MLLMs)~\cite{}, agents based on these predictive models have gained the ability to generate corresponding text-based predictions from given instructions. 

While text-based predictions can provide high-level planning for agents, precise control over an agent's actions requires more detailed predictions. 
%
It has been proposed that \textit{video generation will be to the physical world what language modeling is to the digital world}~\cite{yang2024video}, demonstrating that video-based predictions have a smaller domain gap relative to the action space compared to language~\cite{}. 
%
This allows for more accurate guidance of agents in generating executable actions.
%
Such advanced predictive generative models are referred to as World Simulators, which can simulate realistic experiences based on actions performed by humans and interactive agents. 
%
These World Simulators, particularly those powered by advanced video generative models, are designed to create diverse environments without the need for extensive task-specific customization, while also incorporating robust 3D scene understanding and physical rule priors. 
%
The rapidly evolving field of World Simulators offers exciting opportunities for advancing AGI, with significant potential to enhance human productivity and creativity, especially in the realm of embodied intelligence.


\begin{table}[t]
\centering
\scriptsize
\caption{Comparisons between existing Predictive Model benchmarks. Interactive Environment refers to the interaction with the simulation environment during the prediction phase. Task-Level Interaction denotes the exchanges that occur at the intervals of tasks or subtasks, whereas Action-Level Interaction represents the frequency of interactions that occur through the generation of actions for control purposes.}
\begin{tabular}{@{}lcccccc@{}}
\toprule
Benchmark & Input Modality & Output Modality & Evaluation Level & Interactive Env. & Evaluation Strategy  \\
\midrule
AgentBench & Text & Text & $S_0$ & Task-Level & Embodied Metric   \\
EgoPlan-Bench & Text \& Images & Text & $S_0$ & N/A & PPL~\cite{}   \\
MMWorld & Text \& Images & Text & $S_0$ & N/A & GPT  \\
VAB & Text \& Images & Text & $S_0$ & Task-Level & Embodied Metric  \\
VBench & Text & Video & $S_1$ & N/A & Score-based  \\
EvalCrafter & Text \& Images & Video & $S_2$ & N/A & Score-based  \\
\cmidrule(lr){1-6}
\multirow{2}{*}{\centering \mname} & \multirow{2}{*}{\centering Text \& Images} & \multirow{2}{*}{Actionable Video} & \multirow{2}{*}{\centering $S_3$} & \multirow{2}{*}{\centering Action-Level} & HF-Embodied Evaluator, \\

& & & & & Embodied Metric \\
\bottomrule
\end{tabular}
\end{table}

Although World Simulators have shown tremendous potential in various embodied tasks, the evaluation of their capabilities remains largely unexplored.
%
In this work, we categorize the functionalities of predictive models into a hierarchy ranging from $S_0$ to $S_3$, determined by the types of modalities these models are capable of accepting and producing, as illustrated in Fig.~\ref{fig:motivation}.
% In this work, we categorize predictive models based on human cognition and model capabilities, as illustrated in Fig.~\ref{fig:motivation}.
%
% According to the predictive abilities of generative models, those at the lowest stage, $S_1$, can only generate corresponding text predictions based on control instructions and observations. 
%
This work focuses on models at the $S_3$ stage, also known as World Simulators, a predictive model capable of replicating a vast array of virtual and real-world scenarios. 
%



However, the potential of Video Generation Models as World Simulators remains largely unexplored. 
%
Previous evaluations of generative models [ ] have primarily focused on aesthetic aspects, using traditional core-based methods to assess the quality of generated content. 
%
While this may suffice for creative applications, it fails to comprehensively and accurately evaluate World Simulators that emphasize adherence to physical rules and 3D scene understanding. 
%
In contrast, we argue that an effective evaluation of a World Simulator should adopt a more embodied intelligence perspective. 
%
Specifically, the evaluation criteria should be grounded in aspects relevant to embodied tasks, such as perspective consistency, object breakability, and other physical properties. 
%
These attributes are difficult to accurately capture with core-based methods, but human assessment based on the perceptual quality of generated images often provides a more intuitive and accurate reflection.
%
While perceptual evaluation of these criteria is important, solely relying on aesthetics is insufficient. 
%
We propose that evaluating the capabilities of a World Simulator should also involve the use of inverse dynamics models (IDM) or goal-based models to control embodied agents within the generated videos. 
%
This approach more effectively reflects the World Simulator's ability to adhere to physical rules and manage 3D scenes, as producing accurate control signals requires precise understanding and manipulation of these underlying principles.

We take the very first step in evaluating World Simulators by proposing a hierarchical evaluation framework called \mname. 
%
As shown in Fig.~\ref{fig:motivation} \mname ~assesses World Simulators through two complementary approaches: \textbf{\upstream}, which focuses on the visual quality and condition consistency of generated content, and \textbf{\downstream}, which measures the World Simulator's performance through the conversion of video into control signals. 
%
We present three representative embodied scenarios: \mc(\abmc), \ad(\abad), and \arm(\abarm), to thoroughly evaluate the capability of World Simulators in generating and representing scenario-specific attributes.
%
This approach allows for a thorough assessment of World Simulators across different embodied intelligence tasks, highlighting their strengths and areas for improvement in simulating various real-world interactions.

In the \upstream, we first define evaluation criteria tailored to the unique attributes of each embodied intelligence scenario. 
%
Using these criteria, we construct a comprehensive set of prompts specific to each scenario. 
%
Starting with well-defined meta-types of real-world knowledge, we leverage the capabilities of large language models (e.g., ChatGPT) to expand these meta-prompts into a diverse and extensive set.
%
The prompt lists are then used by various video generation models to produce a large number of video clips.
%
Following extensive human feedback and annotation, these video clips are compiled into the HF-Embodied dataset.
%
Additionally, we train a human preference evaluator using the HF-Embodied dataset to assess World Simulators at the perceptual level, offering a robust evaluation of both their visual fidelity and contextual accuracy.

For the \downstream, we deploy three simulation environments for the three emobodied scenarios respectively: Minecraft for \abmc, CARLA for \abad, and Calvin for \abarm. These environments are used to collect data and train IDM or goal-based policy models capable of mapping future video to actions.
%
In each of these embodied scenarios, the World Simulator is tasked with generating situation-aware videos in real time, based on current observations and provided text instructions.
%
These generated videos are then converted into actions using the pre-trained video-to-action models. 
%
The effectiveness of the World Simulator is implicitly evaluated by measuring the performance of the tasks, using relevant metrics to reflect the quality and accuracy of the generated content.


Our contributions can be summarized as follows:
\begin{itemize}
    \item We introduce the first benchmark for World Simulators, thoroughly evaluating Video Generation Models as World Simulators through a hierarchical assessment framework.
    \item We present the HF-Embodied dataset with corresponding human-like evaluators, enabling comprehensive perceptual evaluation of World Simulators across various embodied scenarios.
    \item During the evaluation, we discuss several insights and findings that may contribute to further innovation and development of video generation models and World Simulators.
\end{itemize}
